Hybrid Physics and Deep Learning Model for Interpretable Vehicle State Prediction

Physical motion models offer interpretable predictions for the motion of vehicles. However, some model parameters, such as those related to aero- and hydrodynamics, are expensive to measure and are often only roughly approximated reducing prediction accuracy. Recurrent neural networks achieve high prediction accuracy at low cost, as they can use cheap measurements collected during routine operation of the vehicle, but their results are hard to interpret. To precisely predict vehicle states without expensive measurements of physical parameters, we propose a hybrid approach combining deep learning and physical motion models including a novel two-phase training procedure. We achieve interpretability by restricting the output range of the deep neural network as part of the hybrid model, which limits the uncertainty introduced by the neural network to a known quantity. We have evaluated our approach for the use case of ship and quadcopter motion. The results show that our hybrid model can improve model interpretability with no decrease in accuracy compared to existing deep learning approaches.

==> table-model_names.tex <==
\setlength{\tabcolsep}{4pt}
\centering
\caption{Abbrevations for evaluated models. Hybrid models consist of a first-principles or a regression component and employ either one- (\texttt{1P}) or two-phase training (\texttt{2P}).}
\label{table:model_names}
\begin{tabular}{@{}ll@{}}
\toprule
Abbrevation & Model \\
\midrule
\texttt{QLag} & \makecell[l]{quadratic control lag (baseline 1, \cite{Punjani2015})}\\[-0.1em]
\texttt{LSTM} & \makecell[l]{stacked LSTM with LSTM initializer\\(baseline 2, \cite{Mohajerin2019})}\\[0.3em]
\texttt{Min-1P/2P} & \makecell[l]{hybrid model with minimal\\first-principles} \\[-0.1em]
\texttt{Pro-1P/2P} & \makecell[l]{hybrid model with propulsion\\first-principles} \\[-0.1em]
\texttt{Lin-1P/2P} & \makecell[l]{hybrid model with linear regression\\(similar to \cite{Woo2018})}\\[-0.1em]
\texttt{Hyd-1P/2P} & hybrid model with hydrodynamic regression \\[0.3em]
\texttt{\{Min,Pro\}+\{Lin,Hyd\}-1P/2P} & \makecell[l]{hybrid model combining first-principles\\and regression}\\
\bottomrule
\end{tabular}


==> table-scores_ship_cis.tex <==
\setlength{\tabcolsep}{5pt}
\centering
\caption{
Root mean squared error and $95\%$-CI for each state variable and trajectory over all test samples.
\texttt{QLag} and \texttt{LSTM} are the physical and DNN baseline respectively.
All other models are hybrid models using one- or two-phase training.
The best and second-best score per column are marked in {\color{RED}red} and {\color{BLUE}blue} respectively.
}
\label{table:rmse}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Model & $u$ & $w$  & $p$ & $r$  & $\phi$ & Trajectory \\[-0.1em]
& [\si{\meter\per\second}] & [\si{\meter\per\second}] & [\si{\radian\per\second}] & [\si{\radian\per\second}] & [\si{\radian}] & [\si{\meter}]\\
\midrule
\texttt{QLag} & 0.098 $\pm$ 0.001 & 0.166 $\pm$ 0.001 & \color{RED}0.0048 $\pm$ 0.0000 & 0.0058 $\pm$ 0.0000 & 0.0210 $\pm$ 0.0001 & 1147 $\pm$ \:9 \\[-0.1em]
\texttt{LSTM} & 0.085 $\pm$ 0.001 & \color{BLUE}0.054 $\pm$ 0.000 & 0.0056 $\pm$ 0.0000 & \color{BLUE}0.0020 $\pm$ 0.0000 & \color{RED}0.0070 $\pm$ 0.0001 & \:290 $\pm$ \:3 \\[0.2em]

\texttt{Min-1P} & 0.112 $\pm$ 0.001 & 0.057 $\pm$ 0.000 & 0.0057 $\pm$ 0.0000 & 0.0025 $\pm$ 0.0000 & 0.0074 $\pm$ 0.0001 & \:385 $\pm$ \:4 \\[-0.1em]
\texttt{Min-2P} & 0.144 $\pm$ 0.001 & 0.070 $\pm$ 0.001 & 0.0059 $\pm$ 0.0000 & 0.0023 $\pm$ 0.0000 & 0.0080 $\pm$ 0.0001 & \:401 $\pm$ \:4 \\[0.2em]

\texttt{Pro-1P} & 0.108 $\pm$ 0.001 & 0.063 $\pm$ 0.000 & 0.0057 $\pm$ 0.0000 & 0.0026 $\pm$ 0.0000 & 0.0079 $\pm$ 0.0001 & \:578 $\pm$ \:5 \\[-0.1em]
\texttt{Pro-2P} & 0.175 $\pm$ 0.001 & \color{BLUE}0.054 $\pm$ 0.000 & 0.0056 $\pm$ 0.0000 & \color{BLUE}0.0020 $\pm$ 0.0000 & 0.0075 $\pm$ 0.0001 & \:317 $\pm$ \:3 \\[0.2em]

\texttt{Lin-1P} & 0.568 $\pm$ 0.004 & 0.645 $\pm$ 0.004 & 0.0072 $\pm$ 0.0001 & 0.0115 $\pm$ 0.0001 & 0.0960 $\pm$ 0.0007 & 1674 $\pm$ 11 \\[-0.1em]
\texttt{Lin-2P} & \color{BLUE}0.077 $\pm$ 0.001 & \color{RED}0.048 $\pm$ 0.000 & 0.0057 $\pm$ 0.0000 & \color{RED}0.0018 $\pm$ 0.0000 & \color{RED}0.0070 $\pm$ 0.0001 & \color{BLUE}\:273 $\pm$ \:3  \\[0.2em]

\texttt{Hyd-1P} &  -- & -- & -- & -- & -- & --\\[-0.1em]
\texttt{Hyd-2P} & 0.084 $\pm$ 0.001 & 0.057 $\pm$ 0.000 & 0.0057 $\pm$ 0.0000 & 0.0021 $\pm$ 0.0000 & \color{BLUE}0.0073 $\pm$ 0.0001 & \:315 $\pm$ \:3 \\[0.2em]

\texttt{Min+Lin-1P} & 0.828 $\pm$ 0.006 & 0.453 $\pm$ 0.003 & \color{BLUE}0.0052 $\pm$ 0.0000 & 0.0169 $\pm$ 0.0001 & 0.0470 $\pm$ 0.0003 & 1575 $\pm$ \:9 \\[-0.1em]
\texttt{Min+Lin-2P} & \color{RED}0.070 $\pm$ 0.001 & 0.055 $\pm$ 0.000 & 0.0060 $\pm$ 0.0000 & \color{BLUE}0.0020 $\pm$ 0.0000 & 0.0074 $\pm$ 0.0001 & \color{RED}\:269 $\pm$ \:3 \\[0.2em]

\texttt{Pro+Lin-1P} & 0.675 $\pm$ 0.005 & 0.500 $\pm$ 0.003 & 0.0056 $\pm$ 0.0000 & 0.0149 $\pm$ 0.0001 & 0.0591 $\pm$ 0.0004 & 1476 $\pm$ \:9 \\[-0.1em]
\texttt{Pro+Lin-2P} & 0.073 $\pm$ 0.001 & 0.063 $\pm$ 0.000 & 0.0062 $\pm$ 0.0000 & 0.0022 $\pm$ 0.0000 & 0.0077 $\pm$ 0.0001 & \:276 $\pm$ \:3 \\[0.2em]

\texttt{Min+Hyd-1P} & 1.667 $\pm$ 0.012 & 0.632 $\pm$ 0.004 & 0.0085 $\pm$ 0.0001 & 0.0143 $\pm$ 0.0001 & 0.0606 $\pm$ 0.0004 & 1798 $\pm$ 10 \\[-0.1em]
\texttt{Min+Hyd-2P} & 0.099 $\pm$ 0.001 & 0.061 $\pm$ 0.000 & 0.0056 $\pm$ 0.0000 & 0.0021 $\pm$ 0.0000 & 0.0077 $\pm$ 0.0001 & \:360 $\pm$ \:3 \\[0.2em]

\texttt{Pro+Hyd-1P} & 0.372 $\pm$ 0.003 & 0.595 $\pm$ 0.004 & 0.0106 $\pm$ 0.0001 & 0.0105 $\pm$ 0.0001 & 0.0892 $\pm$ 0.0006 & 1500 $\pm$ 10 \\[-0.1em]
\texttt{Pro+Hyd-2P} & 0.068 $\pm$ 0.001 & 0.063 $\pm$ 0.000 & 0.0058 $\pm$ 0.0000 & 0.0021 $\pm$ 0.0000 & 0.0078 $\pm$ 0.0001 & \:285 $\pm$ \:3 \\
\bottomrule
\end{tabular}

